Blind Recognition of Touched Keys: Attack and Countermeasures

In this paper, we introduce a novel computer vision based attack that discloses inputs on a touch enabled device, while the attacker cannot see any text or popups from a video of the victim tapping on the touch screen. In the attack, we use the optical flow algorithm to identify touching frames where the finger touches the screen surface. We innovatively use intersections of detected edges of the touch screen to derive the homography matrix mapping the touch screen surface in video frames to a reference image of the virtual keyboard. We analyze the shadow formation around the fingertip and use the k-means clustering algorithm to identify touched points. Homography can then map these touched points to keys of the virtual keyboard. Our work is substantially different from existing work. We target password input and are able to achieve a high success rate. We target scenarios like classrooms, conferences and similar gathering places and use a webcam or smartphone camera. In these scenes, single-lens reflex (SLR) cameras and high-end camcorders used in related work will appear suspicious. To defeat such computer vision based attacks, we design, implement and evaluate the Privacy Enhancing Keyboard (PEK) where a randomized virtual keyboard is used to input sensitive information.

==> background.tex <==
\section{Background}
\label{background}

In this section, we first introduce major computer vision knowledge used in this paper: image formation via projection of a 3D world object into a 2D image and planar homography relation between two images of the same object.
%At last we introduce touch screen technology.

\subsection{Image Formation} \label{secImFormation}
%An object is illuminated by the light source, and it reflects radiation toward camera, then camera senses it via chemicals on the film(image plane). Here, we show the geometry of image formation, showing where point of object's projection locates in the image plane.

Image formation is the process of {\em perspective projection}, projecting 3D points of an object to the image plane of a camera. We use a pin hole camera model to discuss the process. In Figure \ref{imageFormation}, the ray from the 3D point $Q$ passes the optical lens center $O$ and strikes the image plane at $q$. The optical axis $OZ$ is perpendicular to the image plane and the point of interception is called principle point $P$. $OP$ is the focal length.

\begin{figure}[!htp]
\centering
%\vspace{-0.3cm}
\includegraphics[width=2.5in]{imageFormation}\\
%\vspace{-0.3cm}
\caption{Image Formation}
\label{imageFormation}
%\vspace{-0.3cm}
\end{figure}

Given the pin hole camera model Figure \ref{imageFormation}, we can use geometry to describe the mapping between a 3D world object and its image. If we use homogeneous coordinates to represent 2D and 3D points, perspective projection can be represented as linear transform. The homogeneous coordinate of a 3D world point is $\tilde{Q}=\{x, y, z, 1\}^T$ while the corresponding homogeneous coordinate of a pixel image plane point $\tilde{q}=\{x', y', 1\}^T$.
In general, the world and camera coordinate systems are not aligned. We need to find the translation vector $T$ that maps the camera's origin to the world’s origin, and find the rotation matrix $\mathbf{R}$ that aligns the camera’s axes with the world’s axes. $\mathbf{R}$ and $\mathbf{T}$ are called extrinsic camera parameters and form a matrix $\mathbf{\Lambda}$
\begin{equation}
\mathbf{R} = \left[\begin{array}{cc} \mathbf{R}~|~-\mathbf{R}\mathbf{T} \end{array} \right],
\end{equation}
where operator $|$ concatenates the two parts $\mathbf{R}$ and $-\mathbf{R}\mathbf{T}$ into a $3\times4$ matrix.
Once the two coordinate systems are aligned, we can apply perspective transform $\mathbf{C}$ to map a 3D world point onto the image plane and
\begin{equation}\label{exProjection}
  \mathbf{C}=\left(
            \begin{array}{ccc}
              f & 0 & 0 \\
              0 & f & 0 \\
              0 & 0 & 1 \\
            \end{array}
          \right)
\end{equation}
where $f$ is the focal length.
Finally we transform physical image plane coordinates to pixel image plane coordinates via matrix $\mathbf{K}$,
\begin{equation}\label{inProjection}
  \mathbf{K}=\left(
          \begin{array}{ccc}
            1/s_{x} & 0 & o_x \\
            0 & 1/s_{y} & o_y \\
            0 & 0 & 1 \\
          \end{array}
        \right),
\end{equation}
where ($o_x$, $o_y$) is the coordinate of the principal point $P$. $s_x$ and $s_y$ are the actual size of the pixels in the horizontal and vertical directions. Matrices $C$ and $K$ are called intrinsic camera parameters.
In this way,
\begin{equation}\label{world2Image}
\lambda \tilde{q}= \mathbf{K} \mathbf{C} \mathbf{\Lambda} \tilde{Q}
\end{equation}

\subsection{Planar Homography}
\label{homographyTheory}
Planar homography is a 2D projective transformation that relates two images of the same planar object. Points in one image and corresponding points in another image of the same planar object can be mapped by the homography relation. Using the knowledge of image formation, we now introduce planar homography.

For a plane in the 3D world, define
\begin{equation}
\mathbf{U}=\left(
    \begin{array}{cccc}
      a_x & b_x & x_0 \\
      a_y & b_y & y_0\\
      a_z & b_z & z_0 \\
      0 & 0 & 1 \\
    \end{array}
  \right),
\end{equation}
where $(x_0,y_0,z_0)^T$ is the origin of the plane, and $(a_x,a_y,a_z)^T$ and $(b_x,b_y,b_z)$ are the planes direction vectors.
Therefore, given a point in its homogenous form $p=(x', y', 1)^T$ on the plane, we can get the its 3D coordinate $Q=(x, y, z, 1)^T$ by:
\begin{equation}\label{plane2world}
Q = \mathbf{U} p
\end{equation}

According to Equation (\ref{world2Image}), we can derive the 3D point's coordinate in an image plane in the homogeneous form as follows,
\begin{equation}\label{plane2Image}
 q=M_{im} \cdot M_{proj} \cdot M_{ext} \cdot \mathbf{U} . p
=\mathbf{\mathcal{H}}  p
\end{equation}
where $\mathbf{\mathcal{H}} =M_{im} \cdot M_{proj} \cdot M_{ext} \cdot U$ and is an invertible $3\times3$ matrix.

If the point $p=(s, t, 1)$ is projected onto two image planes as $q_1$ and $q_2$ via matrices $\mathbf{\mathcal{H}}_1$ and $\mathbf{\mathcal{H}}_2$ respectively, we have
\begin{equation}
\label{pointINimage1}
  q_1=\mathbf{\mathcal{H}}_1 Q,
\end{equation}
\begin{equation}\label{pointINimage2}
q_2=\mathbf{\mathcal{H}}_2 Q,
\end{equation}
Then
\begin{eqnarray}
q_1 &=& \mathbf{\mathcal{H}}_1 \mathbf{\mathcal{H}}_2^{-1}q_2 \\
    &=& \mathbf{H} q_2
\end{eqnarray}
where $\mathbf{H} = \mathbf{\mathcal{H}} \mathbf{\mathcal{H}}_2^{-1}$ and is an invertible $3\times3$ matrix.

The homography matrix $\mathbf{H}$ has 8 degrees of freedom (Despite 9 entries in it, the common scale factor is not relevant). Therefore, to derive the homography matrix, we just need 4 pairs of corresponding points on the same plane in two imagesm, and any three of them should not be collinear \cite{multiViewGeomerty}.

%\subsection{Touching Screen}
%
%Since this paper uses touch screen as the example for demonstrating our technique, we briefly introduce the ouch screen technology. Currently, there are two types of touching screen technologies \cite{mobileFrontier}: resistive touch screen and capacitive touch screen. They have different structure and ways to sense touching.
%
%A resistive touch screen is composed of two thin, electrically conductive layers separated by a narrow gap. When the screen is touched and pressed by the fingertip or a stylus, the two metallic layers will be connected and causes changes of the electric current, which will be regarded as a touch event. Both touch and pressure are required to trigger a touch event. The touch screen is deformed in the interaction.
%
%\textcolor[rgb]{1.00,0.00,0.00}{A capacitive touch screen is made from glass material with transparent metallic conductive coating.
%An electrode pattern printed along the edges distributes a low voltage field over the conductive layer. When a finger touches
%the screen and draws a minute amount of current to the point of contact, it registers a touch event. Unlike a resistive touchscreen,
%a capacitive touchscreen can be activated with a very light touch,no pressure is required.}
%There is no deformation when touched.
%Even though more expensive than the resistive screen, it responds to touching more quickly. Most mobile touch screen, such as iPad, uses such kind of technology.
%

